YourMT3+: Multi-instrument Music Transcription with Enhanced Transformer Architectures and Cross-dataset Stem Augmentation

Multi-instrument music transcription aims to convert polyphonic music recordings into musical scores assigned to each instrument. This task is challenging for modeling as it requires simultaneously identifying multiple instruments and transcribing their pitch and precise timing, and the lack of fully annotated data adds to the training difficulties. This paper introduces YourMT3+, a suite of models for enhanced multi-instrument music transcription based on the recent language token decoding approach of MT3. We enhance its encoder by adopting a hierarchical attention transformer in the time-frequency domain and integrating a mixture of experts. To address data limitations, we introduce a new multi-channel decoding method for training with incomplete annotations and propose intra- and cross-stem augmentation for dataset mixing. Our experiments demonstrate direct vocal transcription capabilities, eliminating the need for voice separation pre-processors. Benchmarks across ten public datasets show our models' competitiveness with, or superiority to, existing transcription models. Further testing on pop music recordings highlights the limitations of current models. Fully reproducible code and datasets are available with demos at \url{https://github.com/mimbres/YourMT3}.

==> tables/result_ablation.tex <==
\begin{table}[t]
\small
\centering
\begin{tabular}{llll}
\toprule
\it Model & \it Onset F1 & \it Offset F1 & \it Drum F1\\
\midrule
YMT3 base & 64.8 & 41.7 & 77.8 \\
~~~\it{+ Intra-aug.} & +\bf 4.8 & +\bf5.5 & + 0.6\\
~~~\it{+ Full-vocab.} & +0.6 & +2.1 & +2.6\\
~~~\it{+ Data balancing} & + \bf4.0 & +\bf 4.7 & +1.3\\
~~~ & (+2.4*) & (+1.4*) & (+0.3*) \\
~~~\it{+ Cross-aug.} & +\bf 4.7 & +\bf6.8 & +\bf5.2\\
~~~\it{+ PTF-encoder} & +1.8 & +\bf4.2 & +1.9\\
~~~\it{+ MoE FFN} & +1.5 & +\bf4.2 66.75& +1.9 89.51\\
~~~\it{+ Multi decoder} & +1.8 & +\bf4.2 & +1.9\\
\bottomrule
\end{tabular}
\caption{Model component addition analysis. Note onset and offset F1 score (\%) on non-drum instrument classes, and onset F1 score (\%) on drum instrument classes evaluated on Slakh dataset. All models are trained using multiple datasets listed in Table~\ref{tab:comparison} for 400K steps with batch size of 80.  Asterisk ($\ast$) denotes the score achieved by 800K training steps. }
\label{tab:result_ablation}
\end{table}
